Frame-to-Frame Aggregation of Active Regions in Web Videos for Weakly Supervised Semantic Segmentation

When a deep neural network is trained on data with only image-level labeling, the regions activated in each image tend to identify only a small region of the target object. We propose a method of using videos automatically harvested from the web to identify a larger region of the target object by using temporal information, which is not present in the static image. The temporal variations in a video allow different regions of the target object to be activated. We obtain an activated region in each frame of a video, and then aggregate the regions from successive frames into a single image, using a warping technique based on optical flow. The resulting localization maps cover more of the target object, and can then be used as proxy ground-truth to train a segmentation network. This simple approach outperforms existing methods under the same level of supervision, and even approaches relying on extra annotations. Based on VGG-16 and ResNet 101 backbones, our method achieves the mIoU of 65.0 and 67.4, respectively, on PASCAL VOC 2012 test images, which represents a new state-of-the-art.

==> Figure_bargraphs.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{ablation_study_v2.pdf}
  \caption{\label{videoseg_samples} bargraph.}
\end{figure}

==> table_ablations.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tbp]
  \centering
  \caption{Comparison of mIoU scores using different $K$ on PASCAL VOC 2012 validation images. $K=0$ denotes the result trained without web videos.}
    \begin{tabular}{lcccccc}
     \Xhline{1pt}\\[-0.95em]
    K     & 0 & 1     & 2     & 3     & 4     & 5 \\
    \hline\hline
    mIoU  &   61.16 & 62.03    &   62.81    &   -    &   -    & 63.8 \\
     \Xhline{1pt}
    \end{tabular}%
  \label{various_K}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tbp]
  \centering
  \caption{Comparison of mIoU scores using different number of web samples on PASCAL VOC 2012 validation images.}
    \begin{tabular}{lccccccc}
     \Xhline{1pt}\\[-0.95em]
    \# Samples & 0K    &1K & 3K & 5K    & 10K   & 15K   & 18.5K \\
    \hline\hline
    mIoU  &  61.16  &62.49 & 63.18      &63.24  & 63.35    &   63.87  & 63.82 \\
     \Xhline{1pt}
    \end{tabular}%
  \label{n_sample}%
\end{table}%


==> table_video_seg.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Note that our system predict masks for 21 classes, and select corresponding classes. WebCrawl uses binary mask predictor - independt to other classes. }
%   \begin{threeparttable}
% \begin{adjustbox}{max width=0.48\textwidth}
%     \begin{tabular}{lcccc}
%         \Xhline{1pt}

%     method &  sup. & class avg & video avg \\
%     \hline\hline
%     $\text{Tang }\textit{et al.}_{\text{~~CVPR '13}}$~\cite{tang2013discriminative}     &   $\mathcal{U}$& 23.9  & 22.8 \\
%     $\text{Papazoglou }\textit{et al.}_{\text{~~ICCV '13}}$~\cite{papazoglou2013fast}     &  $\mathcal{U}$ & 46.8  & 43.2 \\
%      $\text{Jang }\textit{et al.}_{\text{~~CVPR '16}}$~\cite{jang2016primary}    &  $\mathcal{U}$ & 53.0    & - \\
%     $\text{Zhang }\textit{et al.}_{\text{~~CVPR '15}}$~&$\mathcal{B}$  & 54.1  & 52.6 \\
%      $\text{Drayer }\textit{et al.}_{\text{~~ArXiv '16}}$~\cite{drayer2016object}    &$\mathcal{B}$   & 56.2  & 55.8 \\
%         $\text{Zhang }\textit{et al.}_{\text{~~TPAMI '18}}$~\cite{zhang2018semantic}  &$\mathcal{B}$  & 61.7  & 59.1 \\
%         $\text{Saleh }\textit{et al.}_{\text{~~ICCV '17}}$~ \cite{saleh2017bringing}  &$\mathcal{I}$ & 53.3  & - \\

%      $\text{Hong }\textit{et al.}_{\text{~~CVPR '17}}$~\cite{hong2017weakly}  &$\mathcal{I}$  & 58.6  & 57.1 \\
%     DSRG & &   &  \\

%     Ours  &$\mathcal{I}$ & 62.1 & 57.9\\
%         \Xhline{1pt}

%     \end{tabular}%
%     \end{adjustbox}
%   \label{table_videoseg}%
%   \begin{tablenotes}
%   \footnotesize
%             \item $\mathcal{U}-$Unsupervised, $\mathcal{B}-$Bounding boxes, $\mathcal{I}-$Image labels
%         \end{tablenotes}
%      \end{threeparttable}
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tbp]
  \centering
  \caption{Comparison of video object segmentation methods with various supervision on Youtube-Objects dataset.\\[-2em] }
  \begin{threeparttable}
    \begin{tabular}{lcccc}
        \Xhline{1pt}

    method &  sup. & mIoU  \\
    \hline\hline
    $\text{Tang }\textit{et al.}_{\text{~~CVPR '13}}$~\cite{tang2013discriminative}     &   $\mathcal{U}$& 23.9  \\
    $\text{Papazoglou }\textit{et al.}_{\text{~~ICCV '13}}$~\cite{papazoglou2013fast}     &  $\mathcal{U}$ & 46.8   \\
     $\text{Jang }\textit{et al.}_{\text{~~CVPR '16}}$~\cite{jang2016primary}    &  $\mathcal{U}$ & 53.0     \\
    $\text{Zhang }\textit{et al.}_{\text{~~CVPR '15}}$~\cite{zhang2015semantic}&$\mathcal{B}$  & 54.1   \\
     $\text{Drayer }\textit{et al.}_{\text{~~ArXiv '16}}$~\cite{drayer2016object}    &$\mathcal{B}$   & 56.2   \\
        $\text{Zhang }\textit{et al.}_{\text{~~TPAMI '18}}$~\cite{zhang2018semantic}  &$\mathcal{B}$  & 61.7   \\
        $\text{Saleh }\textit{et al.}_{\text{~~ICCV '17}}$~ \cite{saleh2017bringing}  &$\mathcal{I}$ & 53.3  \\

     $\text{Web-Crawl}_{\text{~~CVPR '17}}$~\cite{hong2017weakly}  &$\mathcal{I}$  & 58.6   \\
     $\text{SROWN}_{\text{~~TIP '18}}$~\cite{yang2018segmentation}  &$\mathcal{I}$  &61.9   \\
    \\[-.95em]\hline\\[-.95em]
    $\text{DSRG}_{\text{~~CVPR '18}}$  \cite{huang2018weakly} & $\mathcal{I}$ &   55.7  \\
$\text{FickleNet}_{\text{~~CVPR '19}}$  \cite{lee2019ficklenet} & $\mathcal{I}$ &   58.2  \\
    Ours  &$\mathcal{I}$ & \textbf{62.1} \\
        \Xhline{1pt}

    \end{tabular}%
  \label{table_videoseg}%
  \begin{tablenotes}
  \footnotesize
            \item $\mathcal{U}-$Unsupervised, $\mathcal{B}-$Bounding boxes, $\mathcal{I}-$Image labels
        \end{tablenotes}
     \end{threeparttable}
\end{table}%

